Numerical Simulation of Gluey Particles

We propose here a model and a numerical scheme to compute the motion of rigid particles interacting through the lubrication force. In the case of a particle approaching a plane, we propose an algorithm and prove its convergence towards the solutions to the gluey particle model proposed by B. Maury. We propose a multi-particle version of this gluey model which is based on the projection of the velocities onto a set of admissible velocities. Then, we describe a multi-particle algorithm for the simulation of such systems and present numerical results.

==> math.tex <==
%pour obtenir le style math\'ematiques
\newcommand{\dsp}{\displaystyle}

\newcommand{\xx}{\mathbf{x}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\xxi}{\mathbf{x}_i}
\newcommand{\xxj}{\mathbf{x}_j}
\def \cancel #1 {}

\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\fb}{\mathbf{f}_B}
\newcommand{\fbi}{\mathbf{f}_{i}}
\newcommand{\oo}{\omega}
\newcommand{\ooi}{\omega_i}
\newcommand{\too}{\tilde\omega}
\newcommand{\tooi}{\tilde\omega_i}
\newcommand{\OO}{\Omega}
\newcommand{\OmB}{{\Omega \setminus \bar{B}}}

\newcommand{\ff}{\mathbf{f}_{\OmB}}

\newcommand{\uu}{\mathbf{u}}
\newcommand{\uueps}{\mathbf{u}_{\varepsilon}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\ww}{\mathbf{w}}
\newcommand{\tuu}{\tilde{\bf u}}
\newcommand{\VV}{\mathbf{V}}
\newcommand{\WW}{\mathbf{W}}
\newcommand{\VVi}{\mathbf{V}_i}
\newcommand{\tVV}{\tilde{\bf V}}
\newcommand{\tVVi}{\tilde{\bf V}_i}
\newcommand{\tUU}{\tilde{\bf U}}
\newcommand{\UU}{\mathbf{U}}
\newcommand{\IR}{\mathbb{R}}
\newcommand{\IN}{\mathbb{N}}
\newcommand{\nn}{\mathbf{n}}
\newcommand{\dB}{\partial B}
\newcommand{\dBi}{\partial B_i}
\newcommand{\dOO}{\partial \OO}
\newcommand{\dOmB}{\partial (\OmB)}
\newcommand{\xo}{\mathbf{x}_0}
\newcommand{\p}{\hbox{p}}
\newcommand{\q}{\hbox{q}}
%\newcommand{\nablat}{^{t}\hspace{-1mm}\nabla}
\newcommand{\nablatu}{(\nabla\uu)^T}
\newcommand{\rhof}{\rho_f}
\newcommand{\rhob}{\rho_B}
\newcommand{\rhobi}{\rho_{i}}
\newcommand{\DuDt}{\frac{\hbox{D}\uu}{\hbox{D}t}}
\newcommand{\DvDt}{\frac{\hbox{D}\vv}{\hbox{D}t}}
\newcommand{\Du}{\mathbf{D}(\uu)}
\newcommand{\Dv}{\mathbf{D}(\vv)}
\newcommand{\Dup}{\mathbf{D}(\uu^{n+1})}
\newcommand{\Dtu}{\mathbf{D}(\tuu)}
\newcommand{\Dun}{\mathbf{D}(\uu_n)}
\newcommand{\Dunbar}{\mathbf{D}(\bar{\uu}_n)}
\newcommand{\unbar}{\bar{\uu}_n}
\newcommand{\Jxo}{\hbox{J}_{\xo}}
\newcommand{\Jxi}{\hbox{J}_{\xxi}}
\newcommand{\Jn}{\hbox{J}^n}
\newcommand{\Jneps}{\hbox{J}^{n}_\varepsilon}
\newcommand{\J}{\hbox{J}}
\newcommand{\Jeps}{\hbox{J}_\varepsilon}
\newcommand{\Kxodiv}{K_{\xo,\nabla}}
\newcommand{\Kxo}{K_{\xo}}
\newcommand{\intOmB}{\int_{\OmB}}
\newcommand{\intdOmB}{\int_{\dOmB}}
\newcommand{\intdB}{\int_{\dB}}
\newcommand{\intdBi}{\int_{\dBi}}
\newcommand{\intOO}{\int_{\OO}}
\newcommand{\intdOO}{\int_{\dOO}}
\newcommand{\intB}{\int_{B}}
\newcommand{\intBi}{\int_{B_i}}
\newcommand{\llambda}{{\boldsymbol\lambda}}
\newcommand{\lambdaij}{{\lambda}_{ij}}
\newcommand{\ksi}{{\boldsymbol\xi}}
\newcommand{\ksiij}{{\xi}_{ij}}
\newcommand{\ggamma}{{\boldsymbol\gamma}}
\newcommand{\gammaij}{{\gamma}_{ij}}
\newcommand{\GG}{\mathbf{G}}
\newcommand{\GGij}{\mathbf{G}_{ij}}
\newcommand{\qq}{\mathbf{q}}
\newcommand{\qqi}{\mathbf{q}_i}
\newcommand{\qqj}{\mathbf{q}_j}
\newcommand{\FF}{{\bf F}}
\newcommand{\bb}{{\bf b}}
\newcommand{\hqqeps}{{\bf q}^\varepsilon}
\newcommand{\huueps}{{\bf u}^\varepsilon}
\newcommand{\hueps}{{u}^\varepsilon}
\newcommand{\hweps}{{w}^\varepsilon}
\newcommand{\hqeps}{{q}^\varepsilon}
\newcommand{\eps}{\varepsilon}
\newcommand{\B}{\mathbf{B}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\ONE}{\mathbf{1}}

\def \SPp {L^2(\OO)}  % espace en pression
\def \XX {{\bf X}}
\def \YY {{\bf Y}}

%espaces fonctionnels
\newcommand{\Ldeux}{{L^2(]a,b[)}}
\newcommand{\Lun}{{L^1(]a,b[)}}
\newcommand{\Linf}{{L^\infty(]a,b[)}}
\newcommand{\Hun}{{H^1(]a,b[)}}
\newcommand{\Hunzero}{{H^1_0(]a,b[)}}
\newcommand{\LunLun}{{L^1(]0,T[\times ]a,b[)}}
\newcommand{\LdeuxLdeux}{{L^2(]0,T[\times ]a,b[)}}
\newcommand{\LunLdeux}{{L^1(]0,T[,L^2(]a,b[))}}
\newcommand{\LunLinf}{{L^1(]0,T[,L^\infty(]a,b[))}}
\newcommand{\LinfLun}{{L^\infty(]0,T[,L^1(]a,b[))}}
\newcommand{\LinfLdeux}{{L^\infty(]0,T[,L^2(]a,b[))}}
\newcommand{\LinfLinf}{{L^\infty(]0,T[\times ]a,b[)}}
\newcommand{\HunHun}{{H^1(]0,T[\times ]a,b[)}}
\newcommand{\Dprim}{{{\cal D}'(]0,T[\times ]a,b[)}}
\newcommand{\LdeuxHun}{{L^2(]0,T[,H^1(]a,b[))}}
\newcommand{\LinfHun}{{L^\infty(]0,T[,H^1_0(]a,b[))}}
\newcommand{\LinfHmun}{{L^\infty(]0,T[,H^{-1}(]a,b[))}}
\newcommand{\HmunHmun}{{H^{-1}(]0,T[\times]a,b[)}}

%convergence faible \'etoile
\newcommand{\wsto}{\stackrel{\star}{\relbar\joinrel\rightharpoonup}}

\newcommand{\vseq}{\vspace{6pt}}
\newcommand{\virg}{,\,\,\,}
\newcommand{\ppt}{\hbox{pour pt}t}

